Enabling Real-time Neural Recovery for Cloud Gaming on Mobile Devices

Cloud gaming is a multi-billion dollar industry. A client in cloud gaming sends its movement to the game server on the Internet, which renders and transmits the resulting video back. In order to provide a good gaming experience, a latency below 80 ms is required. This means that video rendering, encoding, transmission, decoding, and display have to finish within that time frame, which is especially challenging to achieve due to server overload, network congestion, and losses. In this paper, we propose a new method for recovering lost or corrupted video frames in cloud gaming. Unlike traditional video frame recovery, our approach uses game states to significantly enhance recovery accuracy and utilizes partially decoded frames to recover lost portions. We develop a holistic system that consists of (i) efficiently extracting game states, (ii) modifying H.264 video decoder to generate a mask to indicate which portions of video frames need recovery, and (iii) designing a novel neural network to recover either complete or partial video frames. Our approach is extensively evaluated using iPhone 12 and laptop implementations, and we demonstrate the utility of game states in the game video recovery and the effectiveness of our overall design.

==> motivation.tex <==
%\section{Motivation}
%\label{sec:motivation}
%
%In this section, we analyze 4G, 5G, and WiFi traces to understand how well existing networks can support cloud gaming. 

% Time series of delay across 4G, 5G, WiFi (static, moving)

% Time series of loss across 4G, 5G, WiFi  (including those that didn't make the deadline) (static, moving)

% loss percentage (static, moving)


\subsection{Unity Background}
Unity~\cite{unity} is a cross-platform game engine developed by Unity Technologies, which is primarily used to develop video games and simulations for computers, consoles and mobile devices. The rendering pipeline in Unity involves a combination of shader calculations, textures, surface treatments, the viewer’s perspective, and lighting.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/unity.pdf}
    \vspace{-20pt}
    \caption{Simplified Rendering Process in Unity}
    \vspace{-5pt}
    \label{fig:unity_rendering_process}
\end{figure}

Fig.~\ref{fig:unity_rendering_process} shows a simplified rendering process in Unity. A renderer consists of meshes, textures, and shaders. A mesh describes the geometry of a game object, and is represented using vertices and multiple triangle arrays. Each game object has at least one texture, which determines its color and transparency. The shader is a program that computes the color of each pixel according to the lighting and material. 

\para{Culling: } For each frame, a camera performs frustum culling to remove renderers that fall outside the camera's view. In addition, occlusion culling further removes the objects that are occluded. Both frustum culling and occlusion culling remove the need of rendering unnecessary objects, and enhance efficiency. 

% When the rendering starts, the CPU goes through the scene’s renderer components and adds them to a list. Each mesh has a bounding box that is converted into an AABB per renderer and CPU checks those against the frustum of the camera. Any renderers whose bounds are not visible will be skipped and removed from the list. CPU also compares the layer mask on the camera against the renderers and skips those that are not visible. Then CPU checks if this is the first time any of renderers have been seen, and if so it uploads them to GPU.

\para{Setup Rendering: } Next CPU will sort renderer components, such as render queue, materials, lighting, depth, etc. For example, the depth sorting can be used to separate transparent and opaque objects. After uploading the data to GPU, CPU needs to set up the shared data that is not going to change between objects, \eg, the camera’s world to view transform and projection matrices. Along with the shared data, all the required data of game objects, such as local to world transform matrix, the textures, the mesh data, the shaders, and the effect state like the blend mode, front or back face culling are sent to GPU to start rendering. 

\para{Vertex Shader: } When GPU receives the uploaded data, it will start the vertex shader, where each vertex position of a game object is transformed from the local space to homogeneous clip space in parallel. The vertex shader also optionally modifies or passes on any extra data, like the UVs and color. 

\para{Rasterization: } GPU goes through the index array and calculates the screen coverage for each triangle based on the vertex positions. This is done in the order they exist in the array and not in parallel. If a triangle covers any pixels on screen, the depth buffer will be updated. Otherwise, the triangle will be skipped and invisible. Then GPU starts drawing the pixels for that triangle. For each pixel it needs to calculate the barycentric coordinate, and interpolate the vertex data to pass on to that pixel’s fragment shader. 

\para{Fragment Shader: } The fragment shader is usually used to calculate and output the color of each pixel. Pixels on screen are processed in batches and in parallel. Textures are sampled with specialized hardware that handles fast decoding and filtering of the various texture formats and splits out a color value for the shader to use. The fragment shader takes the interpolated data for every triangle’s position, as well as any of the material properties and texture data, and puts them together to form a single color value.

\subsection{Local Rendering}

When the network condition gets worse during cloud gaming, the most straightforward approach to recover lost frames is to perform rendering at the client side, namely, local rendering. To quantify the feasibility of this approach, we measure the resource usage and achieved FPS when rendering some high-quality games on the two following local machines. 
\begin{itemize}
    \item Laptop: Intel(R) Core(TM) i7-8650U CPU @ 1.90GHz   2.11 GHz; Nvidia GeForce GTX 1050 (2GB).
    \item Desktop: Intel(R) Xeon(R) CPU E3-1271 v3 @ 3.60GHz; Nvidia GeForce GTX 1050 Ti (4GB).
\end{itemize}

Viking Village~\cite{vk}, Corridor
~\cite{nature} and Nature~\cite{corridor} are high-quality virtual-world Unity apps with complex and realistic environments as shown
in Figure~\ref{fig:games}. Since these games are originally designed for high-end PCs, we use them for our experiment.  

\begin{figure*}[htpb]
  \centering
  \subfigure[Viking Village]{%
    \includegraphics[width=0.5\columnwidth]{figures/vk.png}
    \vspace{-20pt}
    \label{fig:vk}
  }
  \subfigure[Nature]{%
    \includegraphics[width=0.5\columnwidth]{figures/nature.png}
    \vspace{-20pt}
    \label{fig:nature}
  }
  \subfigure[Corridor]{%
    \includegraphics[width=0.5\columnwidth]{figures/corridor.png}
    \vspace{-20pt}
    \label{fig:corridor}
  }
  \subfigure[Viking Village+]{%
    \includegraphics[width=0.5\columnwidth]{figures/vk+.png}
    \vspace{-20pt}
    \label{fig:vk+}
  }
  \caption{High-quality Unity games.}
  \vspace{-10pt}
  \label{fig:games}
\end{figure*}

The results in Table~\ref{tab:FPS} show that the three high-quality games, Viking Village, Corridor
and Nature are achieved only 19-25 FPS, which makes the local rendering not promising on the laptop. The desktop has a more powerful CPU and GPU, leading to providing more than 30FPS for these three games. However, the games used for cloud gaming might be more complex and time-consuming for rendering. Given that, we build a bigger game based on Viking Village by enlarging the game area and putting more game objects to the scene. The bigger game is called Viking Village+. From Table~\ref{tab:FPS}, the desktop can only support Viking Village+ with 15FPS.        

In summary, our experiment suggests that local machines suffer a rendering delay of 40-66ms because of the heavy rendering workload for high-quality games. Therefore, we have to seek other ways to recover the lost frames.  

\begin{table}
  \caption{FPS when running different high-quality games}
  \vspace{-10pt}
  \label{tab:FPS}
  \begin{tabular}{ccc}
    \toprule
    Machine & Game Name & FPS \\
    \midrule
    \multirow{3}{*}{Laptop} & Viking Village & 21  \\
    & Nature & 25 \\
    & Corridor & 19 \\ \hline
    \multirow{1}{*}{Desktop} & Viking Village+ & 15  \\
    \bottomrule
  \end{tabular}
\end{table}
